The sixth Painleve transcendent and uniformizable orbifolds

We consider connection between the Painleve-6 equation and explicitly uniformizable orbifolds

==> MACRO+.tex <==
% ! Следующие команды корректно работают только
% при \usepackage{hyperref}, так как только при hyperref можно
% явно устанавливать \paperwith, \textwidth
\usepackage{hyperref}
% \textcenter: Указать размеры текста (включая колонтитулы),
% задать запись в верхний колонтитул
% и разместить все по центру листа (его размеры не меняются)

% \textcenter{0mm}{0mm} - оставить размеры как установлено в cls-файле
\newcommand{\textcenter}[3][Yu.~Brezhnev]{
\pagestyle{myheadings}% задаем текст в колонтитуле
\markboth{\hfill\textsc{#1}\hfill}{\hfill\textsc{#1}\hfill}
% центруем по ширине
\ifdim#2=0mm\textwidth=\textwidth\else\textwidth=#2\fi
% !Такой способ присваивания работает только в преамбуле
\oddsidemargin=\paperwidth%
\addtolength{\oddsidemargin}{-\textwidth}%
\addtolength{\oddsidemargin}{-2in} \oddsidemargin=0.5\oddsidemargin
\evensidemargin=\oddsidemargin
% центруем по высоте
\ifdim#3=0mm\textheight=\textheight\else\textheight=#3\fi
\topmargin=\paperheight%
\addtolength{\topmargin}{-\textheight}%
\addtolength{\topmargin}{-2in}%
\addtolength{\topmargin}{-\headsep}%
\addtolength{\topmargin}{-\headheight}%
\addtolength{\topmargin}{-\footskip}%
\topmargin=0.5\topmargin}

% \obrezka: Обрезать лист, т.е. задать \pagewidth, \pageheight,
% так, чтобы текст (его размеры не меняются) был окружен заданными
% полями слева|справа|сверху

\newcommand\obrezka[2]{
\oddsidemargin=#1 \paperwidth=\textwidth%
\addtolength{\paperwidth}{2\oddsidemargin}%
\addtolength{\oddsidemargin}{-1in} \evensidemargin=\oddsidemargin%
\topmargin=#2 \paperheight=\textheight%
\addtolength{\paperheight}{\headsep}%
\addtolength{\paperheight}{\headheight}%
\addtolength{\paperheight}{\footskip}%
\addtolength{\paperheight}{2\topmargin}%
\addtolength{\topmargin}{-1in}}

